Repeatability Is Not Enough: Learning Affine Regions via Discriminability

A method for learning local affine-covariant regions is presented. We show that maximizing geometric repeatability does not lead to local regions, a.k.a features,that are reliably matched and this necessitates descriptor-based learning. We explore factors that influence such learning and registration: the loss function, descriptor type, geometric parametrization and the trade-off between matchability and geometric accuracy and propose a novel hard negative-constant loss function for learning of affine regions. The affine shape estimator -- AffNet -- trained with the hard negative-constant loss outperforms the state-of-the-art in bag-of-words image retrieval and wide baseline stereo. The proposed training process does not require precisely geometrically aligned patches.The source codes and trained weights are available at https://github.com/ducha-aiki/affnet

==> wbsori.tex <==
\begin{table*}[htb]
\ra{1.15}
\centering
%\small
\caption{Comparison of the local features orientation estimators on wide baseline stereo with Hessian and adaptive Hessian detectors, following the protocol~\cite{WXBS2015} on wide baseline stereo datasets. Number of matched image pairs and average number of inliers are reported. Numbers is the header corresponds to the number of image pairs in dataset. We don`t highlight best results, as they are nearly identical for all methods.}
\begin{tabular}{lrrrrrrrrrrrr}
\toprule
& \multicolumn{2}{c}{EF~\cite{Zitnick2011}}
& \multicolumn{2}{c}{EVD~\cite{MODS2015}}
& \multicolumn{2}{c}{OxAff~\cite{Mikolajczyk2005}}
& \multicolumn{2}{c}{SymB~\cite{Hauagge2012}}
& \multicolumn{2}{c}{GDB~\cite{Yang2007}}
%& \multicolumn{2}{c}{map2photo}
& \multicolumn{2}{c}{LTLL~\cite{Fernando2015}}
\\
\cmidrule(r){2-3}
\cmidrule(r){4-5}
\cmidrule(r){6-7}
\cmidrule(r){8-9}
\cmidrule(r){10-11}
\cmidrule(r){12-13}
%\cmidrule(r){14-15}
Detector
 & 33& inl.
 & 15& inl. 
 & 40& inl.
 & 46& inl.
 & 22& inl.
% & 6& inl.
 & 172& inl.\\
\cmidrule(r){1-13}
DomOri\cite{SIFT2004} &33 & 97 &2 & 30 &40 & 1070 &35 & 181 &19 & 190&36 & 36 \\
ONetPosNeg &33 & 96 &3 & 27 &40 & 1058 &36 & 175 &19 & 189&36 & 35 \\
ONetPos &33 & 96 &3 & 27 &40 & 1058 &36 & 176 &19 & 188&37 & 34 \\
OriNet~\cite{OriNet2016} &33 & 96 &2 & 31 &40 & 1050 &35 & 178 &19 & 186&37 & 34 \\
\cmidrule(r){1-13}
DomOriMulti~\cite{SIFT2004} &33 & 116 &2 & 52 &40 & 1181 &38 & 208 &19 & 233 &46 & 38\\
\bottomrule
\end{tabular}
%\vspace{1em}
\label{tab:wbs-ori}
\end{table*}
